Gradientless Descent: High-Dimensional Zeroth-Order Optimization

Zeroth-order optimization is the process of minimizing an objective $f(x)$, given oracle access to evaluations at adaptively chosen inputs $x$. In this paper, we present two simple yet powerful GradientLess Descent (GLD) algorithms that do not rely on an underlying gradient estimate and are numerically stable. We analyze our algorithm from a novel geometric perspective and present a novel analysis that shows convergence within an $\epsilon$-ball of the optimum in $O(kQ\log(n)\log(R/\epsilon))$ evaluations, for any monotone transform of a smooth and strongly convex objective with latent dimension $k < n$, where the input dimension is $n$, $R$ is the diameter of the input space and $Q$ is the condition number. Our rates are the first of its kind to be both 1) poly-logarithmically dependent on dimensionality and 2) invariant under monotone transformations. We further leverage our geometric perspective to show that our analysis is optimal. Both monotone invariance and its ability to utilize a low latent dimensionality are key to the empirical success of our algorithms, as demonstrated on BBOB and MuJoCo benchmarks.

==> nodelta_proof.tex <==
%!TEX ROOT=aistats2019.tex
\subsection{Proof without Delta}

\renewcommand{\y}{y}
\newcommand{\z}{z}
% \begin{proof}
% Let $\y_{t-1}, \y_t$ be the point closes to $x^*$ in the level set $\levelset_{t-1}, \levelset$, respectively.
% Let
% $w_t$ be the point that $\levelset_{t}$ and the ray from $x^*$ to $\y_{t-1}$ intersect, and
% $w_{t-1}$ be the point that $\levelset_{t-1}$ and the ray from $x^*$ to $\y_{t}$ intersect.
% \[1 - \frac{\|w_{t} - x^*\|}{\|\y_{t-1} - x^*\|} = \frac{\|w_{t-1} - \y_t\|}{\|w_{t-1} - x^*\|} \geq \frac{1}{Q^2}\frac{\|b_{t-1} - q\|}{\|b_{t-1} - x^*\|}
% = \frac{1}{5dQ^3}\]

% So, $\|\y_{t} - x^*\| \leq (1 - \frac{1}{5dQ^3}) \|y_{t-1} - x^*\|$.
% \end{proof}


\begin{lemma}
Define $\Phi_t = \diam{\mathcal{X}}\paren{\decayfactor}^t.$
Then, $\|b_t - x^*\| \leq \Phi_t$ for all $t$ with probability $\eta$.
\end{lemma}
\begin{proof}
Clearly, $\bd{0} \leq \Phi_0$. Now suppose $\|\bd{t-1} - x^*\| \leq \Phi_{t - 1}$ for induction.

Let $z_t = \arg\max_{x: f(x) = f(b_t)} \|x - x^*\|$ be the point in $\levelset_{b_t}$ that is maximally far from $x^*$.

Let $q = \paren{\decayfactor}\bp_{t-1} + \frac{1}{5d\Q} \point^*$.
Let $B_q = \cB(c_q, r_q)$ be ball contained in $\levelset_q$ such that $q$ is on its surface; the existence of $B_q$ is guaranteed by Lemma~\ref{lem:enclosed_ball}.
\newcommand{\LLval}{Q^{-1}(1-\nu)}
\newcommand{\UUval}{\nu + Q^{-1}(1-\nu)}
\newcommand{\LL}{L}
\newcommand{\UU}{U}

Let $\nu = \nuval.$
Note that $\nu \leq 1/5$ for any $\Q, \dim \geq 1$.
So,
\begin{equation}
\label{eq:good_event:1}
\textstyle
  \nu Q(1-\nu)^{-1} = \frac{1}{5\dim}(1 - \nu)^{-1}\leq \frac{1}{4\dim}.
\end{equation}

Let $\ell = \|b_{t-1} - c_q\|$. Note that $\ell \leq \|b_{t-1} - q\| + r_q
\leq \nu \|b_{t-1} - x^*\| + r_q
= \nu \|b_{t-1} - x^*\| + Q^{-1}\|q - x^*\|
= \nu \|b_{t-1} - x^*\| + Q^{-1}(1-\nu)\|b_{t-1} - x^*\|$
Also, $\ell \geq r_q = Q^{-1}\|q - x^*\| = Q^{-1}(1-\nu)\|b_{t-1} - x^*\|$, because $b_{t-1}$ is outside $B_q$.

Let $\LL = \LLval$ and $\UU = \UUval$, so that $\LL \bd{t-1} \leq \ell \leq \UU \bd{t-1}.$ Note that
\begin{equation}
  \frac{\UU}{\LL} = 1 + \nu Q(1-\nu)^{-1} = 1 + \frac{1}{5\dim}(1 - \nu)^{-1}
\leq 1 + \frac{1}{4 \dim} \leq \frac{5}{4}
\end{equation}
and
\begin{equation}
\frac{L}{U} \leq \decayfactor
\end{equation}

for all $\dim, Q \geq 1.$

\textbf{Case 1:} Suppose $\Phi_{t-1} > \frac{\UU}{\LL} \|z_{t-1} - x^*\|$. Then, $ \|z_{t-1} - x^*\| < \frac{\LL}{\UU}\Phi_{t-1} \leq (1-\frac{1}{5 \dim Q^3}) \Phi_{t-1} = \Phi_t$ and therefore
 \[\|z_{t} - x^*\| \leq \|z_{t-1} - x^*\| \leq  \Phi_{t}.\]

% \textbf{Case 2:} Suppose $\LL\|b_{t-1} - x^*\| \leq \LL\Phi_{t-1} \leq \UU \|b_{t-1} - x^*\|$.
% Note that $\ell$ also belongs to this interval and $\frac{\LL}{\UU} \geq \frac{4}{5}$. If $\hat{\ell}\leq \ell$, then $\hat{\ell} \geq \frac{4}{5} \ell \geq ell/2.$ Otherwise, $\ell \leq \hat{\ell}$ but $\ell \geq  \frac{4}{5}\hat{\ell}$ and also, $\ell/2 \leq \frac{4}{5}\ell \leq \frac{4}{5}\hat{\ell}$. Therefore,
%  at least one of $\hat{\ell}$ or $\frac{4}{5}\hat{\ell}$ is in $[\ell/2, \ell]$.
% %Proof by mathematica: http://www.wolframalpha.com/input/?i=Solve%5Bq%5E-1+(1-+(1%2F(5+d+q)))+%2F+((1%2F(5+d+q))+%2B+(1-(1%2F(5+d+q)))+%2F+q)+%3C%3D+1+-+(1%2F(5+d+q))+q%5E-2%5
% So, $\|y_{t} - x^*\| \leq \Phi_{t} \|y_{t-1} - x^*\| \leq \Phi_{t} \|b_{t-1} - x^*\|$

\textbf{Case 2:} Suppose $\Phi_{t-1} \leq \frac{\UU}{\LL} \zd{t-1}$.
By Lemma~\ref{lem:prelim:radius_ratio}, it follows that $\Phi_{t-1} \leq \frac{\UU}{\LL}\sqrt{Q} \bd{t-1}$.
Note that \[\frac{\ell}{2} \leq \frac{\UU}{2}\bd{t-1} \leq \LL\bd{t-1} \leq \ell \leq \UU \bd{t - 1}.\]
If there exists $r_{k, i} \in [\frac{1}{2}\UU\bd{t-1}, \UU \bd{t-1}]$,
then we can apply Lemma~\ref{lem:ball-intersection}.
It suffices to note that $\log_2 \frac{\sqrt{Q}}{\LL} \leq \log_2 \frac{5}{4} Q^{\frac{3}{2}} \leq \frac{3}{2} \log_2 Q + \log_2\frac{5}{4}.$



Take $L\Phi_t$ and divide by $\log(\UU / \LL)$ each time up to $\log \sqrt{Q} / \log (\UU / \LL)$ times. Then,
\[L\Phi_t / \sqrt{Q} \leq  U\|b_{t-1} - x^*\|\]
and at least one value should lie in $[L\|b_{t-1} - x^*\|, U\|b_{t-1} - x^*\|]$.

% So, the algorithm would try $\frac{U}{L}^{K} (L\Phi_{t-1}, \frac{4}{5}L\Phi_{t-1})$ for $k = 1, \ldots, \log_{\frac{U}{L}}Q$ each round.

% $\log \frac{U}{L} \geq \log(1 + \frac{1}{5dQ}) > \frac{1}{5dQ} - \frac{1}{50d^2Q^2} \geq \frac{1}{5dQ} - \frac{1}{200}$ So, $(\log \frac{U}{L})^{-1} \leq 6 d Q$ for all $d \geq 2, Q \geq 1$. So,
% we make $12d Q \log Q$ evaluations per trial.

Each trial has the success rate of at least $0.25$. Therefore, by repeating $\log_{.75}\eta T^{-1} = \frac{\log (\eta^{-1} T)}{\log \frac{4}{3}} \leq 4 \log (\eta^{-1} T)$ trials per epoch, each epoch fails with $\eta T^{-1}$ probability. By the union bound over $T$, this failure is only $\eta$. Condition on the probability that every epoch succeded. The above
induction gives after $T$ epochs,
\[\exp\paren{-\frac{T}{5dQ^3}}\|z_0 - x^*\|\]
\end{proof}

In terms of evaluations (points to evaluate),
\[\exp\left(-\frac{T}{300 d^2Q^4 \log Q \log (\eta^{-1} T)}\right)\|z_0 - x^*\|\]


==> old_theorems.tex <==
\begin{lemma}
\label{lem:prelim:radius_ratio}
  If $h$ has condition number $Q$, then for all $b \in  \levelset_a(h)$,
  \[\textstyle Q^{-\frac{1}{2}} \leq \frac{\|a - x^*\|}{\|b-x^*\|} \leq Q^{\frac{1}{2}}.\]
\end{lemma}
\begin{proof}
  Write $h = g \circ f$ as in the above proof.
  We first prove the lower bound:
  \setlength{\jot}{8pt}   % Extra space between the aligned lines.
  \begin{align*}
    \min_{y \in h(\mathcal{X})} \min_{\substack{h(a) =y \\ h(b) = y}} \frac{\|a - x^*\|}{\|b - x^*\|}
    &=     \min_{y \in f(\mathcal{X})} \min_{\substack{f(a) =g^{-1}(y) \\ f(b) = g^{-1}(y)}} \frac{\|a - x^*\|}{\|b - x^*\|} \\
    &\geq \min_{y \in f(\mathcal{X})} \frac{\min_{a : f(a) = y}\|a - x^*\|}{\max_{b: f(b) = y}\|b - x^*\|} \\
    &\geq \sqrt{\frac{\frac{y - f(x^*)}{\alpha}}{\frac{y - f(x^*)}{\beta}}} = \sqrt{\frac{\beta}{\alpha}}
  \end{align*}
  The proof for the upper bound follows the same logic, with denominators and numerators swapped.
\end{proof}

Our last lemma shows that regardless of which direction we converge to $x^*$, the rate of convergence is not much different.
\begin{lemma}
\label{lem:balanced}
Let $f$ be a function with condition number $Q$. Let $x_1, y_1 \in \X$ such that $x_1 \leq \sublevelset_{y_1}$ and $x_1$ is on the line between $x^*$ to $y_1$. Let $x_2 \in \levelset_{x_1}$ and $y_2 \in \levelset_{y_1}$ such that $x_2$ is on the line between $x^*$ to $y_2$.
See the diagram below for the visualization of this setup. Then, 
\[Q^{-2} \leq \frac{\frac{\|y_1 - x_1\|}{\|y_1-x^*\|}}{\frac{\|y_2 - x_2\|}{\|y_2-x^*\|}} \leq Q^2.\]
\end{lemma}
\begin{center}
\includegraphics[width=.38\textwidth]{figs/level_sets.png}
\end{center}
  % https://www.geogebra.org/graphing/eauuwxxy
\begin{proof}
% It follows that
% \[\min_{\substack{a,a',b,b' \in \mathrm{Im}(f) \\ f(a) = f(a') < f(b) = f(b')}}
% \frac{\frac{\|a - x^*\|}{\|b - x^*\|}}{\frac{\|a' - x^*\|}{\|b' - x^*\|}}
% \geq \min_{a,a'}\frac{\|a - x^*\|}{\|a' - x^*\|} \min_{b,b'}\frac{\|b' - x^*\|}{\|b - x^*\|}
% \geq \frac{\alpha}{\beta}.
% \]
Let $r_i = \|x_i - x^*\|$ and $s_i = \|y_i - x_i\|.$
Define 
\[\textstyle f_i(t) = f\left(x^* + t\frac{x_i - x^*}{\|x_i - x^*\|}\right).\]
Then, $f_i'(t) =
\left\langle \nabla f\big(x^* + t\frac{x_i - x^*}{\|x_i - x^*\|}\big), \frac{x_i - x^*}{\|x_i - x^*\|}\right\rangle$ and $f_i''(t) = \frac{x_i - x^*}{\|x_i - x^*\|}^\top \nabla^2 f\big(x^* + t\frac{x_i - x^*}{\|x_i - x^*\|}\big) \frac{x_i - x^*}{\|x_i - x^*\|}$.
Note that $f_i'(t) = 0$ and by strong convexity and smoothness,
  $\alpha \leq f_i''(t) \leq \beta.$
  So,
\begin{align*}
  f_i(r_i + s_i) - f_i(r_i)
  &= \textstyle \int_{r_i}^{r_i + s_i}f'_i(t)\ dt \\
  &= \textstyle \int_{r_i}^{r_i + s_i}f'_i(t) - f'_i(0)\ dt \\
  &= \textstyle \int_{r_i}^{r_i + s_i} \int_{0}^{t} f_i''(s)\ ds \ dt \\
  &\leq \textstyle \int_{r_i}^{r_i + s_i} \int_{0}^{t} \beta \ ds \ dt \\
&= \beta(r_is_i + s_i^2/2)
\end{align*}
and similarly, $f_i(r_i + s_i) - f_i(r_i) \geq \alpha(r_is_i + s_i^2/2)$.
Therefore,
\begin{align*}
  &\frac{\alpha}{2}s_2^2 + \alpha r_2 s_2
  \leq f_2(r_2 + s_2) - f_2(r_2) \\
  =& f_1(r_1 + s_1) - f_1(r_1) \leq \frac{\beta}{2} s_1^2 + \beta r_1 s_1
\end{align*}
  Write $s_2 = k s_1$. Because $\beta \geq \alpha, k \geq 1$.
  Apply the above inequality together with the bound $r_1 \leq \sqrt{\frac{\beta}{\alpha}} r_2$ (Lemma~\ref{lem:prelim:radius_ratio}) to obtain:
\[\frac{\alpha}{2}k^2 s_1^2 + \alpha r_2 k s_1 \leq \frac{\beta}{2} s_1^2 + \beta r_1 s_1
\leq \frac{\beta}{2} s_1^2 + \beta\sqrt{\frac{\beta}{\alpha}} r_2 s_1 \]
By solving for $k$, we have % (proof by wolfram)
% http://www.wolframalpha.com/input/?i=Solve%5Bb+s%5E2+%2B+2+b+*+Sqrt%5Bb+%2F+a%5D+r+s+%3D%3D+a+k%5E2+s%5E2+%2B+2+a+r+k+s,k%5D
\begin{align*}
  1 \leq k &\leq \textstyle \frac{\sqrt{\alpha^2r_2^2 + 2 \alpha \beta r_2 s_1 \sqrt{\frac{\beta}{\alpha}} + \alpha \beta s_1^2} - \alpha r_2}{\alpha s_1} \\
  &\leq \textstyle\frac{\sqrt{\left(\alpha r_2 + \beta\sqrt{\frac{\beta}{\alpha}} s_1 \right)^2} - \alpha r_2}{\alpha s_1} \leq (\beta/\alpha)^{\frac{3}{2}}
\end{align*}
It follows that $s_2 \leq (\beta/\alpha)^{\frac{3}{2}} s_1$.
To complete the proof, note that $r_2 + s_2 \geq \sqrt{\frac{\alpha}{\beta}}(r_1 + s_1)$ by Lemma~\ref{lem:prelim:radius_ratio}.
% Therefore,
% $\frac{s_2}{r_2 + s_2} \leq \frac{\beta^2}{\alpha^2}\frac{s_1}{r_1 + s_1}$.
% http://www.wolframalpha.com/input/?i=Reduce%5B1+%3C+(-a+r+%2B+sqrt(a%5E2+r%5E2+%2B+2+a+b+sqrt(b%2Fa)+r+s+%2B+a+b+s%5E2))%2F(a+s)+%3C+(b%2Fa)%5E(3%2F2),+0%3Ca%3Cb,+r%3E%3D0%5D
\end{proof}


\section{The Gradientless Descent Algorithms} \label{sec:algorithm}

In this section, we present two algorithms that follow the same Gradientless Descent (GLD) template but have slightly different tradeoffs between having better convergence bounds and requiring fewer assumptions. The QGLD (Algorithm~\ref{alg:q}) has a stronger convergence guarantee of order $\exp(-S/\log S)$ (where $S$ is the number of function evaluations) but requires an upper bound on the condition number of the objective function; the $\res$GLD (Algorithm~\ref{alg:delta}) has a weaker convergence guarantee of order $\exp(-\sqrt{S})$ in the best case, but requires no information about the objective function.

The GLD template is as follows; we start at $b_0$ and at iteration $t$, we sample $y_t$ from a uniform distribution over a ball (or balls) around $b_{t-1}$. If $f(y_t) < b_{t-1}$, then update $b_{t} = y_{t}$ and otherwise, we set $b_t = b_{t-1}$. This template is very simple to implement and efficient to run. In addition, unlike the zeroth-order algorithms that compute gradients from function evaluations, we do not require any division by a small number, which makes our algorithm more numerically stable.

As we mentioned before, the key to fast convergence is the careful choice of step sizes, which we describe in full detail in Theorem~\ref{thm:decay_probability}.
The intuition here is that we would like to take as large steps as possible while keeping the probability
of improving the objective function reasonably high.
% we can find a step size such that a random step direction has a good chance of significantly improving the function value.

The main challenge in proving convergence is that because we do not assume strong convexity or Lipschitz continuity of $f$, it is difficult to measure the rate of progress based on the function values only;
even if $f(b_t) - f(x^*)$ is very large, $\|b_t - x^*\|$ may be arbitrarily small. Interestingly, 
our algorithms trivially guarantee that $f(b_t) \leq f(b_{t-1})$, but it is not always the case that $\bd{t} \leq \bd{t-1}$.
This is why we introduce a potential function
\[
\pot(x) := \paren{\max \set{\xd{x}: x \in \levelset_{x}}}
\]
and its shorthand notation $\pot_t := \pot(b_t)$.
Clearly, $\pot_{t}$ is an upper bound on $\bd{t}$ and it is non-increasing in $t$.
% Our convergence rates (in Section~\ref{sec:proofs}) give an upper bound on $\frac{\Phi_t}{\Phi_0}$.

As a technical note, we require that $\X \supseteq \levelset_{b_0}$. This means that $f$ must be well-defined over $\sublevelset_{b_0}$, or $b_0$ must be known to be sufficiently far away from the boundaries.
% he concept of the diameter $\|\X\|$ is a bit  elusive for our algorithms which may try to evaluate functions at arbitrary points in $\R^\dim$. For us, if $d$ is the maximum distance between $b_0$ and $x^*$, then we require the function to be well-defined on $\X =  \{x \in \R^\dim: \|x - x^*\| \leq Q\|b_0 - x^*\|\}$ and that is our radius.


\subsection{Step Size}


We show that given both upper and lower bounds on $\norm{b_t - x^*}$, a good step size can always be found among a small set of candidates. 
% Using this step size will make a significant improvement in the potential function with a reasonably high probability.
\begin{theorem}
\label{thm:decay_probability}
Suppose $\frac{3}{5Q}\xd{x} \in [C_1, C_2]$ for some numbers $C_1, C_2 \in \R^+$. Then, there exist integers $0 \leq k_1, k_2 < \log\frac{C_2}{C_1}$ such that if $r = 2^{k_1} C_1$ or $r = 2^{-k_2} C_2$, then a random sample $y$ from uniform distribution over $B_x = \cB(x, \frac{r}{\sqrt{\dim}})$ satisfies
\[\textstyle \Phi(y) \leq \Phi(x) \paren{\decayfactor} \]
with probability at least $\frac{1}{4}$.
 % Let $R =\{r: r \leq C_2$ \text{ and } $r=2^k C_1$ for some non-negative integer $k\}$, or $R = \{r: r \geq C_1$ \text{ and } $r=2^{-k} C_2$ for some non-negative integer $k\}$. Then, there exists $r \in R$ such that
\end{theorem}
Proving the above theorem requires the following lemma, which is proved in the appendix.
\begin{lemma}
\label{lem:ball-intersection}
  Let $B_1$ and $B_2$ be two balls in $\R^\dim$ of radii $r_1$ and $r_2$ respectively.
  Let $\dc$ be the distance between the centers.
  If $r_1 \in [\frac{\dc}{2\sqrt{\dim}}, \frac{\dc}{\sqrt{\dim}}]$ and
  $r_2 \ge \dc - \frac{\dc}{4 \dim}$, then
  \[
   \vol{B_1 \intersect B_2} \geq c_\dim \vol{B_1},
  \]
  where $c_\dim$ is a dimension-dependent constant that is lower bounded by $\ballconst$ at $\dim = 1$ and converges to $1$ as $\dim$ goes to infinity.
\end{lemma}

\begin{center}
\includegraphics[width=.40\textwidth]{figs/improvements.png}
\end{center}


\begin{proof}(of Theorem~\ref{thm:decay_probability}) Since there are a lot of notations in this proof, we included the above diagram as a visual aid.
% , and $y$ be a random sample from uniform distribution over $B_x$.

Let $\nu = \frac{1}{5\dim\Q}$.
% Note that $\nu \leq 1/5$ for any $\Q, d \geq 1$.
Let $q = (1-\nu)\xx + \nu \point^*$.
Let $B_q = \cB(c_q, r_q)$ be a ball that has $q$ on its surface, lies inside $\sublevelset_q$, and has radius $r_q = Q^{-1}\|x - x^*\|$. Lemma~\ref{lem:enclosed_ball} guarantees its existence.

Suppose that 
\begin{equation}
\label{eq:decay_probability:bal}
\textstyle \vol{B_x \cap B_q} \geq \frac{1}{4} \vol{B_x}    
\end{equation}
and that a random sample $y$ from $B_x$ belongs to $B_q$, which happens with probability at least $\frac{1}{4}$. Then, $\Phi(y) \leq \Phi(q)$.

Let $z_x, z_{q}$ be a point in $\sublevelset_{x}, \sublevelset_{q}$, respectively, that is maximally far away from $x^*.$
% Let $x' = \arg\max_{z \in \sublevelset_{{}f(x)}} \|z - x^*\|$ be a point in $\levelset_y$ that is maximally far away from $x^*$, and similarly define $y'$
% Similarly, define $z_{t-1} \in \levelset_{b_{t-1}}$.
% Let $w_{q}$ be the point in $\levelset_{q}$ such that $w_{q} - x^* = \mu(x - x^*)$ for some positive real number $\mu$; in other words, it is where the ray from $x^*$ to $x$ intersects with $\levelset_{q}$. Similarly, 
Let $w_{x} \in \levelset_{x}$ be the point where the ray $x^*$ from $z_{q}$ intersects with $\levelset_{x}$.

By Lemma~\ref{lem:balanced},
\begin{align*}
\textstyle
1 - \frac{\xd{z_{q}}}{\xd{w_x}} = \frac{\norm{w_x - z_q}}{\xd{w_x}}
\geq \frac{1}{Q^2}\frac{\norm{x - q}}{\xd{x}}
= \frac{1}{5\dim Q^3}.
\end{align*}
It then follows that
\begin{equation*}
\textstyle
% \label{eq:delta:1}
 \Phi(y) \leq \Phi(q) = \|z_q - x^*\| \leq \paren{\decayfactor}\|z_x - x^*\|.
\end{equation*}


It now suffices to prove Eq.~\ref{eq:decay_probability:ball}. To do so, we will apply Lemma~\ref{lem:ball-intersection} after showing that the radius of $B_x$ and $B_q$ are in the proper ranges.
Let $\ell = \norm{x - c_q}$ and note that
\begin{align}
\ell &\leq \|\xx - q\| + r_q \label{eq:ell_rq}\\
&\leq \nu \xd{\xx} + r_q  = \nu \xd{\xx} + Q^{-1} \xd{q} \notag \\
&\leq \textstyle (\nu + Q^{-1}(1-\nu))\xd{x} \label{eq:ell_lx} \\
&\leq \textstyle \frac{6}{5Q}\bd{x} \notag.
% &\leq \textstyle  \label{eq:ell_lq}
\end{align}
Since $\xx$ is outside of $B_q$, we also have
\begin{align}
\ell &\geq r_q = Q^{-1}\xd{q} = Q^{-1}(1-\nu)\xd{\xx} \notag \\
& \textstyle \geq \frac{4}{5Q}\bd{x}. \label{eq:ell_ux}
\end{align}
% Define shorthand notations $\LL = \LLval$ and $\UU = \UUval$, so that we can write $\LL \xd{\xx} \leq \ell \leq \UU \xd{\xx}.$

It follows that
\[\frac{\ell}{2} \leq \frac{3}{5Q}\bd{x}  \leq \ell.\]
In the $\log_2$ space, our choice of $k_1$ is equivalent to starting from $\log_2 C_1$ and sweeping through the range $[\log_2 C_1, \log_2 C_2]$ at the interval of size 1. This is guaranteed to find a point between $\frac{\ell}{2}$ and $\ell$, which is also an interval of size 1. Therefore, there exists a $k_1$ satisfying the theorem statement, and similarly, we can prove the existence of $k_2$.

Finally, it remains to show that \(r_q \geq (1 - 1/(4 \dim))\ell.\)
From Eq. \eqref{eq:ell_rq}, it suffices to show that $\|x - q\| \leq \frac{\ell}{4\dim}$ or equivalently $\nu\xd{\xx} \leq \frac{\ell}{4\dim}$. From Eq. \eqref{eq:ell_lx},
\[\|x - q\| = \nu \xd{\xx} \leq \nu Q(1-\nu)^{-1}\ell.\]
For any $\Q, \dim \geq 1$, $1 - \nu \geq \frac{4}{5}$. So,
\begin{equation}
\label{eq:good_event:1}
\textstyle
  \nu Q(1-\nu)^{-1} = \frac{1}{5\dim}(1 - \nu)^{-1}\leq \frac{1}{4\dim}
\end{equation}
and the proof is complete.
\end{proof}

\subsection{Gaussian Sampling (HI I AM NEW)}
A direct application of Lemma~\ref{lem:ball-intersection} seems to imply that uniform sampling of a high-dimensional ball is necessary. Upon further inspection, the lemma relies on a very simple variance calculation and can be easily replaced with a much simpler Gaussian sampling procedure that concentrates the mass closer to the surface to the ball. As we will see later, this procedure lends itself to better analysis in the high-dimensional regime.

\begin{lemma}
\label{lem:gaussian-intersection}
  Let $B_1$ and $B_2$ be two balls in $\R^\dim$ of radii $r_1$ and $r_2$ respectively.
  Let $\dc$ be the distance between the centers.
  If $r_1 \in [\frac{\dc}{2\sqrt{\dim}}, \frac{\dc}{\sqrt{\dim}}]$ and
  $r_2 \ge \dc - \frac{\dc}{4 \dim}$ and $X = (X_1, ..., X_n)$ are independent Gaussians with mean centered at the center of $B_1$ and variance $\frac{r_1^2}{\dim}$, then
  \[
   \prob{X \in B_2 } > c_\dim,
  \]
  where $c_\dim$ is a dimension-dependent constant.
\end{lemma}

\begin{proof}
Without loss of generality, let $\dc = 1$ and $B_2$ is centered at the origin with radius $r_2$ and $B_1$ is centered at $e_1 = (1, 0, ..., 0)$. Then, we simply want to show that 
$$\prob{(1+X_1)^2 + \sum_{i=2}^\dim X_i^2 \leq r_2^2  } > c_\dim $$

Since it is a chi-squared variable, by standard concentration inequalities, we see that $\sum_{i=2}^\dim X_i^2 \leq O(r_1^2) = O(1/\dim)$ with constant probability. And since $r_2 \geq 1 - O(1/\dim)$, it suffices to show that 

$$\prob{(1+X_1)^2 \leq 1 - O(1/\dim)  } > \Omega(1) $$

Since $X_1$ has standard deviation at least $r_1/\sqrt{n} \geq 1/(2n)$, we see that the probability of deviating at least 1 standard deviation below is at least a constant.
\end{proof}

Note that Lemma~\ref{lem:gaussian-intersection} allows us to simplify our ball-sampling procedure to use Gaussians, rather than the more cumbersome uniform sampling. More importantly, our sampling allows us to exploit any low-dimensional structure that $f(x)$ has. Assume that there exists some rank $k$ matrix $A$ such that $f(x) = g(Ax)$, where $k$ is much smaller than $\dim$. Because Gaussians projected on a $k$-dimensional subspace are still Gaussians, we show that our algorithm has a dimension dependence on $k$.  

\begin{theorem}
\label{thm:decay_lowdim}
Let $f(x) = g(Ax)$ for some unknown rank $k$ matrix $A$ with $k < \dim$. Suppose $\frac{3}{5Q}\xd{x} \in [C_1, C_2]$ for some numbers $C_1, C_2 \in \R^+$. Then, there exist integers $0 \leq k_1, k_2 < \log\frac{C_2}{C_1}$ such that if $r = 2^{k_1} C_1$ or $r = 2^{-k_2} C_2$, then a random sample $y$ from uniform distribution over $B_x = \cB(x, \frac{r}{\sqrt{k}})$ satisfies
\[\textstyle \Phi(y) \leq \Phi(x) \paren{1 - \frac{1}{5kQ^3}} \]
with probability at least $\Omega(1)$.
 % Let $R =\{r: r \leq C_2$ \text{ and } $r=2^k C_1$ for some non-negative integer $k\}$, or $R = \{r: r \geq C_1$ \text{ and } $r=2^{-k} C_2$ for some non-negative integer $k\}$. Then, there exists $r \in R$ such that
\end{theorem}
\begin{proof}
We can consider the projection of all points onto the column space of $A$ and since the Gaussian sampling process is preserved, our proof follows from that of Theorem~\ref{thm:decay_probability} restricted onto the $k$-dimensional subspace.
\end{proof}

Note that the speed-up in progress is due to the fact that we can now tolerate the larger sampling radius of $r/\sqrt{k}$, while maintaining a high probability of making progress. If $k$ is unknown, we can simply use binary search to find the correct radius with an extra factor of $\log(n)$ in our runtime. 

(TO ADD HERE?)
Consider $f(x) = g(\PA x ) + \delta h(x)$. Let $Q_g$ be the condition number of $g$ and $\beta_g, \alpha_g$ be defined similarly. Let $x^*$ be the optima of $g$ such that $\PA x^* = x^*$
\subsection{\texorpdfstring{$Q$}{Q}-Gradientless Descent}


\begin{algorithm}[t]
\SetKwBlock{Ballsample}{Ball Sampling:}{end}
\SetKwInOut{Input}{Input}
\caption{$Q$-Gradientless Descent (QGLD) \label{alg:q}}
  \Input{function $\obj: \R^\dim \to \R$, \\
  $\overline{Q}$: upper bound on $f$'s condition number, \\
  $S \in \Z_+$: max number of evaluations of $f$, \\
  $\eta \in (0, 1)$: acceptable failure probability \\
  $\bp_0$: starting point}
  Set $K = \textstyle\floor{\frac{3}{2} \log_2 \overline{Q} + \log_2\frac{5}{4}}$ \\
  % Set $K = \ceil{\frac{3}{2} \log_2 \overline{Q} + \log_2\frac{5}{4}} \leq 2(\log_2 \overline{Q} + 1)$. \\
  Choose $T$ so that $T \log \eta^{-1}T \leq S$. \\
  \For{t = 1, \ldots, T}{
  Update $R_{t-1} = \diam{\mathcal{X}}\paren{\decayfactorq}^{t-1}$. \\
  \For{$i = 1, \ldots, \max(4 \log(\eta^{-1} T),1)$}{
  \textbf{Ball Sampling Trial $i$:}\\
  \For{k = 0, \ldots, K}{
    Set $r_{i,k} = 2^{-k}R_{t-1} $. \label{alg:q:r}\\
    Sample \uar{\candidate_{i,k}}{\mathcal{B}(\bp_{t-1}, \frac{3}{5\sqrt{\dim}}r_{i,k})}. \\
    % Sample $\uar{\candidate_{i,k}}{B_{i,k}}$, where
    % $B_{i,k} := \set{\point : \norm{x - \bp_{t-1}} \le r_{i,k}}$ \\
    % Set $\point_{i,k}$ to be the projection of $\candidate_{i,k}$ onto $\X$.
  }
  }
  \textbf{Update Step: }
    $\bp_t = \argmin \set{\obj(\point) : \point \in \set{\point_{i, k}} \cup \set{\bp_{t-1}}}.$
  } % End For
\Return{$b_T$}
\end{algorithm}

QGLD (Algorithm~\ref{alg:q}) uses a potential function $R_t$ that upper bounds $\bd{t}$, which we prove  in Lemma~\ref{lem:qgld}.
The lower bound is unknown, but if $\bd{t} \leq R_{t+1}$ already, then it is okay to choose the wrong step size and make no progress for the iteration $t$. So, we use $R_{t+1} \leq \|b_{t} - x^*\| \leq R_{t}$ to search for the step size. 
To guarantee that $R_t$ stays above $\bd{t}$ with high probability for all $t$, we make repeated \emph{trials} for each candidate step size.

\begin{lemma}
\label{lem:qgld}
For QGLD, $\Phi_t \leq R_t$ for all $t$ with probability $1 - \eta$.
\end{lemma}
\begin{proof}
Let $z_t = \arg\max_{x: f(x) = f(b_t)} \|x - x^*\|$ be the point in $\levelset_{b_t}$ that is maximally far from $x^*$.
Clearly, $\zd{0} \leq R_0 = \diam{\X}$. Now suppose $\zd{t-1} \leq R_{t - 1}$ for induction.

% Let $q = \paren{\decayfactor}\bp_{t-1} + \frac{1}{5d\Q} \point^*$.
% Let $B_q = \cB(c_q, r_q)$ be ball contained in $\levelset_q$ such that $q$ is on its surface; the existence of $B_q$ is guaranteed by Lemma~\ref{lem:enclosed_ball}.

% % Let $\nu = \nuval.$

% Let $\ell = \|b_{t-1} - c_q\|$. Note that
% \begin{equation}
%   \frac{\UU}{\LL} = 1 + \nu Q(1-\nu)^{-1} = 1 + \frac{1}{5\dim}(1 - \nu)^{-1}
% \leq 1 + \frac{1}{4 \dim} \leq \frac{5}{4}
% \end{equation}
% and
% \begin{equation}
% \frac{L}{U} \leq \decayfactor
% \end{equation}
% for all $\dim, Q \geq 1.$

If $\|z_{t-1} - x^*\| \leq \paren{\decayfactorq} R_{t-1}$, then we trivially have:
% $ \|z_{t-1} - x^*\| < \frac{\LL}{\UU}R_{t-1} \leq (1-\frac{1}{5 \dim Q^3}) R_{t-1} = R_t$ and therefore
 \(\bd{t} \leq \|z_{t} - x^*\| \leq \|z_{t-1} - x^*\| \leq  R_{t}.\)
%
% \textbf{Case 2:} Suppose $\LL\|b_{t-1} - x^*\| \leq \LL\Phi_{t-1} \leq \UU \|b_{t-1} - x^*\|$.
% Note that $\ell$ also belongs to this interval and $\frac{\LL}{\UU} \geq \frac{4}{5}$. If $\hat{\ell}\leq \ell$, then $\hat{\ell} \geq \frac{4}{5} \ell \geq ell/2.$ Otherwise, $\ell \leq \hat{\ell}$ but $\ell \geq  \frac{4}{5}\hat{\ell}$ and also, $\ell/2 \leq \frac{4}{5}\ell \leq \frac{4}{5}\hat{\ell}$. Therefore,
%  at least one of $\hat{\ell}$ or $\frac{4}{5}\hat{\ell}$ is in $[\ell/2, \ell]$.
% %Proof by mathematica: http://www.wolframalpha.com/input/?i=Solve%5Bq%5E-1+(1-+(1%2F(5+d+q)))+%2F+((1%2F(5+d+q))+%2B+(1-(1%2F(5+d+q)))+%2F+q)+%3C%3D+1+-+(1%2F(5+d+q))+q%5E-2%5
% So, $\|y_{t} - x^*\| \leq \Phi_{t} \|y_{t-1} - x^*\| \leq \Phi_{t} \|b_{t-1} - x^*\|$
%
So, it suffices to consider the case
\[\textstyle \zd{t-1} \geq \paren{\decayfactorq} R_{t-1}.\]
By Lemma~\ref{lem:prelim:radius_ratio}, $\zd{t-1} \leq \sqrt{Q} \bd{t-1} \leq \sqrt{\overline{Q}}\bd{t-1}$.
% it follows that $R_{t-1} \leq \paren{\decayfactor}\sqrt{Q} \bd{t-1}$.
Combined with our inductive hypothesis,
\(\textstyle \paren{\decayfactorq}\frac{1}{\sqrt{\overline{Q}}}R_{t-1} \leq \|b_{t-1} - x^*\| \leq R_{t-1}\)
and hence,
\[\textstyle \paren{\decayfactorq}\frac{1}{\overline{Q}\sqrt{\overline{Q}}}R_{t-1} \leq \frac{\|b_{t-1} - x^*\|}{Q} \leq R_{t-1}.\]
%
Our iteration over $k =0,\ldots, K$ sweeps through this range at an interval of size 1 in the $\log_2$ space, and combined with the multiplication in line \ref{alg:q:r}, it makes Theorem~\ref{thm:decay_probability} applicable.
Thus, each \emph{trial} has $\frac{1}{4}$ probability of producing a candidate for $b_t$ which would guarantee that
\begin{equation}
  \label{eq:qgld_induction}
  \textstyle
  \zd{t} \leq \paren{\decayfactor}R_{t-1} = R_t.
\end{equation}
%
By repeating $\log_{.75}\eta T^{-1} = \frac{\log (\eta^{-1} T)}{\log \frac{4}{3}} \leq 4 \log (\eta^{-1} T)$ trials, each epoch $t=1,\ldots,T$ fails to produce any candidate for $b_t$ to make Equation~\ref{eq:qgld_induction} hold with at most $\eta T^{-1}$ probability. By the union bound, this failure probability is at most $\eta$ over all epochs. So, the induction is valid with probabilty at least $1- \eta$.
\end{proof}
%
It follows that QGLD achieves the convergence rate of $O(\exp(-S / \log S))$.
 % where $S$ is the number of function evaluations.
\newcommand{\nuvalue}[0]{\ensuremath{\frac{\theta}{5 \dim}}}
\newcommand{\balnuvalue}[0]{\ensuremath{\frac{1}{5dQ^3}}}
\newcommand{\pevent}{\ensuremath{\rho}}
\begin{theorem}
Suppose that $\overline{Q}$ is no less than the condition number of $f$. Then, the output $b_T$ of QGLD satisfies with probability at least $1 - \eta$,
\[\textstyle \Phi(b_T) \leq \Phi(b_0) \exp\paren{-\frac{S}{40\dim \overline{Q}^3(\log_2 \overline{Q} +1)\log (\eta^{-1} S)}}.\]
\end{theorem}
If the upper bound $\overline{Q}$ is loose, then $R_t$ stays well above $\bd{t}$. As a result, QGLD tries to take very large steps that are unlikely to lead to any improvement.
On the other hand, if $\overline{Q} < Q$, then $R_t$ decreases faster than $\bd{t}$ and our algorithm will try to take small steps that are more likely to improve but only by a small amount. In practice, such slow but steady progress may be more desirable than all-or-zero progress, but our proof technique treat all small improvements below a certain threshold as zero improvement.


\subsection{\texorpdfstring{$\res$}{r}-Gradientless Descent}
\begin{algorithm}[t]
\SetKwBlock{Ballsample}{Ball Sampling Step:}{end}
\SetKwInOut{Input}{Input}
\caption{$\res$-GradientLess Descent ($\gamma$GLD) \label{alg:delta}}
  \Input{function $\obj: \R^\dim \to \R$, \\
  $T \in \Z_+$: number of evaluations of $f$, \\
  $\eta \in (0, 1)$: acceptable failure probability,  \\
  $\bp_0$: starting point, \\
  $\res$: resolution of the convergence}
  Set $K = \floor{\log{\frac{\|\X\|}{\res}}}$ and $R = \set{\frac{3}{5}\res \cdot 2^k : 0 \le k \le K}$ \\
  \For{$t = 1, \dots, T$}{
    Sample $\uar{r_t}{R}$ \\
    Sample $\uar{\candidate_t}{\cB(\bp_{t-1}, \frac{1}{ \sqrt{\dim}}r_t)}$.
    % , where
    % $B_t := \set{\point : \norm{x - \bp_{t-1}} \le r_t}$.
  % Set $\point_t$ to be the projection of $\candidate_t$ onto $\X$. \\
      %  Select $\point_t = \proj_{\X}\paren{\hat{\point}}$ to be the
      % projection of $\hat{\point}$ onto $\X$
\\
  \textbf{Update:}
    $\bp_t = \argmin \set{\obj(\point) : \point \in \set{\bp_{t-1}, \point_t}}$
     } % End For
\Return{$b_t$}
\end{algorithm}
$\res$GLD (Algorithm~\ref{alg:delta}) does not require any information about the objective function. Instead, it takes a resolution parameter $\res$ as input and its convergence guarantee only holds up to $Q \res$.
% This is more desirable in practice, because it is hard to obtain a tight upper bound on the condition number, and rather than fixing the number of evaluations, we often want to converge within a fixed error.
In other words, $\res$ is a lower bound on $\bd{t-1}/Q$ while the algorithm is still converging. For the upper bound, we use the trivial bound $\|\X\|$. 
% The main advantage of $\res$GLD over QGLD is that it does not require any information about the condition number as input, and the algorithm will still converge exponentially towards $Q \res$.

A big difference is that since $\res$GLD has no potential function to maintain, it is enough to take one random sample per iteration. Each iteration has a low probability of improving the function value significantly, but when we aggregate over a large number of iterations, we obtain a high probability bound.


\begin{theorem}
\label{thm:convergence_delta}
With probability at least $1 - \eta$, Algorithm~\ref{alg:delta} returns a point $b_T$ such that $\bd{T} \leq \epsilon$ after $O(nQ^3 \log(\|\X\|/\epsilon)^2)$ function evaluations.
\end{theorem}

\begin{proof}


\end{proof}

The following theorem is somewhat misleading. Consider using the above theorem


\begin{theorem}
\label{thm:convergence_delta}
If $Q$ is the condition number of $f$, then with probability at least $1 - \eta$,
  \begin{equation*}
\bd{T} \le \max \paren{Q\res,
      \Phi_0 \paren{\decayfactor}^{\Lambda_T}
%      - \frac{\pevent (T-1) \bal \theta}{\dim \numradii}
%      + \sqrt{2 (T - 1) \balnuvalue \ln \paren{2 / \eta}}
        }
  \end{equation*}
where $\Lambda_T = \frac{T}{4 \log_2\paren{|\X| / \res}} - \sqrt{2 T \log \eta^{-1}}$.
\end{theorem}
% The above theorem shows that the algorithm converges exponentially towards $Q\res$.
% When the upper bound for $Q$ is known, we can optimize for $\res$ and $\res$GLD achieves the convergence rate of $O(\exp(-\sqrt{S}))$ where $S$ is the number of function evaluations, which is asymptotically slower than QGLD.
% \begin{corollary}
%  \label{thm:convergence_delta_Q}
%  Suppose there is an upper bound $\overline{Q}$ on the condition number of $f$.
%  Let $c = \log 2 / \log \paren{\decayfactorq}$ and set
% \[\gamma = \diam{\X}\paren{\decayfactorq}^{c\sqrt{\frac{T}{2\log\eta^{-1} + 2 c}}}.\]
% Then, the output $b_T$ of $\gamma$GLD satisfies
% \(\Phi(b_T) \leq Q\gamma\)
% % \exp\paren{-\frac{S}{40\dim Q^3(\log_2 Q +1)\log (\eta^{-1} S)}}\]
% with probability at least $1 - \eta$.
% \end{corollary}
\newcommand{\LLval}{Q^{-1}(1-\nu)}
\newcommand{\UUval}{\nu + Q^{-1}(1-\nu)}
\newcommand{\LL}{L}
\newcommand{\UU}{U}
  \newcommand{\azumavar}{}
  \newcommand{\az}{\ensuremath{z}}  % Quanity for Azuma's ineq.
% \begin{lemma}
% \label{lem:high_probability_bound}
% Suppose $f$ is a monotone transformation of a convex function with condition number $Q$. Then with probability at least $1-\eta,$
%   \begin{equation*}
%     { \bd{T} \le \max \paren{Q\res,
%       \Phi_0 \paren{\decayfactor}^{\Lambda_T}
% %      - \frac{\pevent (T-1) \bal \theta}{\dim \numradii}
% %      + \sqrt{2 (T - 1) \balnuvalue \ln \paren{2 / \eta}}
%         }
%       }
%      \end{equation*}
% where $\Lambda_T = \frac{T}{\log_2\paren{|\X| / \res}} - \sqrt{2 T \ln \eta^{-1}}$.
% \end{lemma}
  \begin{proof}
  Define $\Delta_t = \log_{\decayfactor}\frac{\Phi_{t}}{\Phi_{t-1}}$. Then, $\pot_T = \pot_0 \exp(\sum_{t=1}^T \Delta_T)$ and the theorem is a high-probability bound on the random variable $\Delta_{1:T} := \sum_{t=1}^T \Delta_t$. In order to apply concentration bounds, we define a bounded version of $\Delta_t$ as follows:
  \[
    \hdelta_t =
  \begin{cases}
    -1& \text{if $\Delta_t \leq -1$} \\
    0            & \text{otherwise.}
  \end{cases}
  \]
  Because our potential function never increases, $\Delta_t \leq \hdelta_t$ and
  it now suffices to upper bound the random variable $\hdelta_{1:T} := \sum_{t=1}^T \hdelta_t$.

  If $\bd{t} < Q\res$ for any $t \leq T$, then the statement is trivially true. So, assume $\bd{t} \geq Q\res$ for all $t$. Then, $\res \leq \frac{\bd{t}}{Q} \leq \diam{\X}$.
  Our choice of $R$ sweeps through this range with a unit-sized interval in the $\log_2$ space. Hence, we can apply Theorem~\ref{thm:decay_probability} and conclude there is at least $\frac{1}{4(K + 1)}$ probability that $\Delta_t \leq -1.$

 It immediately follows that
 \(\textstyle \expct{\hdelta_{1:T}} \ \le \ -\frac{T}{4 (K + 1)}.\)
  % \begin{split}
  % \expct{\hdelta_{1:T}} \le & -\sum_{t=1}^T \balnuvalue \pevent_t / \numradii \\
  % \le & -\frac{\pevent (T) \bal \theta}{\dim \numradii}
  % \end{split}
  % \end{equation*}
  Finally, we apply Azuma's inequality:
  \begin{equation} \label{eq:azuma1}
  \prob{ \hdelta_{1:T} - \expct{\hdelta_{1:T}} \geq \az }
  \le \exp \paren{-\frac{\az^2}{2T}}.
  \end{equation}
  To complete the proof, set
  $\az = \sqrt{2 T \log \eta^{-1}}$.
  \end{proof}
If we set $\res$ to be of order $\exp(-\sqrt{T}/\diam{\X})$, then $\Phi_T$ is of order $Q \exp\paren{-\frac{\sqrt{T} \log \eta^{-1}}{5\dim Q^3}}.$


\begin{figure*}[t]
    \includegraphics[width=\textwidth]{figs/qs.png}
    \caption{The average optimality gap by the condition number of the objective function.}
    \label{fig:bigq}
\end{figure*}

\begin{figure*}[t]
  \includegraphics[width=\textwidth]{figs/dims.png}
  \includegraphics[width=\textwidth]{figs/laplace.png}
\caption{The average optimality gap on a quadratic objective function that is strongly convex and smooth objective (top); and its monotone transformation (bottom). See the main text for details.\label{fig:by_dim}}
\end{figure*}

\subsection{\texorpdfstring{$Q$}{Q}-Gradientless Descent}


\begin{algorithm}[t]
\SetKwBlock{Ballsample}{Ball Sampling:}{end}
\SetKwInOut{Input}{Input}
\caption{$Q$-Gradientless Descent (QGLD) \label{alg:q}}
  \Input{function $\obj: \R^\dim \to \R$, \\
  $\overline{Q}$: upper bound on $f$'s condition number, \\
  $S \in \Z_+$: max number of evaluations of $f$, \\
  $\eta \in (0, 1)$: acceptable failure probability \\
  $\bp_0$: starting point}
  Set $K = \textstyle\floor{\frac{3}{2} \log_2 \overline{Q} + \log_2\frac{5}{4}}$ \\
  % Set $K = \ceil{\frac{3}{2} \log_2 \overline{Q} + \log_2\frac{5}{4}} \leq 2(\log_2 \overline{Q} + 1)$. \\
  Choose $T$ so that $T \log \eta^{-1}T \leq S$. \\
  \For{t = 1, \ldots, T}{
  Update $R_{t-1} = \diam{\mathcal{X}}\paren{\decayfactorq}^{t-1}$. \\
  \For{$i = 1, \ldots, \max(4 \log(\eta^{-1} T),1)$}{
  \textbf{Ball Sampling Trial $i$:}\\
  \For{k = 0, \ldots, K}{
    Set $r_{i,k} = 2^{-k}R_{t-1} $. \label{alg:q:r}\\
    Sample \uar{\candidate_{i,k}}{\mathcal{B}(\bp_{t-1}, \frac{3}{5\sqrt{\dim}}r_{i,k})}. \\
    % Sample $\uar{\candidate_{i,k}}{B_{i,k}}$, where
    % $B_{i,k} := \set{\point : \norm{x - \bp_{t-1}} \le r_{i,k}}$ \\
    % Set $\point_{i,k}$ to be the projection of $\candidate_{i,k}$ onto $\X$.
  }
  }
  \textbf{Update Step: }
    $\bp_t = \argmin \set{\obj(\point) : \point \in \set{\point_{i, k}} \cup \set{\bp_{t-1}}}.$
  } % End For
\Return{$b_T$}
\end{algorithm}

QGLD (Algorithm~\ref{alg:q}) uses a potential function $R_t$ that upper bounds $\bd{t}$, which we prove  in Lemma~\ref{lem:qgld}.
The lower bound is unknown, but if $\bd{t} \leq R_{t+1}$ already, then it is okay to choose the wrong step size and make no progress for the iteration $t$. So, we use $R_{t+1} \leq \|b_{t} - x^*\| \leq R_{t}$ to search for the step size. 
To guarantee that $R_t$ stays above $\bd{t}$ with high probability for all $t$, we make repeated \emph{trials} for each candidate step size.

\begin{lemma}
\label{lem:qgld}
For QGLD, $\Phi_t \leq R_t$ for all $t$ with probability $1 - \eta$.
\end{lemma}
\begin{proof}
Let $z_t = \arg\max_{x: f(x) = f(b_t)} \|x - x^*\|$ be the point in $\levelset_{b_t}$ that is maximally far from $x^*$.
Clearly, $\zd{0} \leq R_0 = \diam{\X}$. Now suppose $\zd{t-1} \leq R_{t - 1}$ for induction.

% Let $q = \paren{\decayfactor}\bp_{t-1} + \frac{1}{5d\Q} \point^*$.
% Let $B_q = \cB(c_q, r_q)$ be ball contained in $\levelset_q$ such that $q$ is on its surface; the existence of $B_q$ is guaranteed by Lemma~\ref{lem:enclosed_ball}.

% % Let $\nu = \nuval.$

% Let $\ell = \|b_{t-1} - c_q\|$. Note that
% \begin{equation}
%   \frac{\UU}{\LL} = 1 + \nu Q(1-\nu)^{-1} = 1 + \frac{1}{5\dim}(1 - \nu)^{-1}
% \leq 1 + \frac{1}{4 \dim} \leq \frac{5}{4}
% \end{equation}
% and
% \begin{equation}
% \frac{L}{U} \leq \decayfactor
% \end{equation}
% for all $\dim, Q \geq 1.$

If $\|z_{t-1} - x^*\| \leq \paren{\decayfactorq} R_{t-1}$, then we trivially have:
% $ \|z_{t-1} - x^*\| < \frac{\LL}{\UU}R_{t-1} \leq (1-\frac{1}{5 \dim Q^3}) R_{t-1} = R_t$ and therefore
 \(\bd{t} \leq \|z_{t} - x^*\| \leq \|z_{t-1} - x^*\| \leq  R_{t}.\)
%
% \textbf{Case 2:} Suppose $\LL\|b_{t-1} - x^*\| \leq \LL\Phi_{t-1} \leq \UU \|b_{t-1} - x^*\|$.
% Note that $\ell$ also belongs to this interval and $\frac{\LL}{\UU} \geq \frac{4}{5}$. If $\hat{\ell}\leq \ell$, then $\hat{\ell} \geq \frac{4}{5} \ell \geq ell/2.$ Otherwise, $\ell \leq \hat{\ell}$ but $\ell \geq  \frac{4}{5}\hat{\ell}$ and also, $\ell/2 \leq \frac{4}{5}\ell \leq \frac{4}{5}\hat{\ell}$. Therefore,
%  at least one of $\hat{\ell}$ or $\frac{4}{5}\hat{\ell}$ is in $[\ell/2, \ell]$.
% %Proof by mathematica: http://www.wolframalpha.com/input/?i=Solve%5Bq%5E-1+(1-+(1%2F(5+d+q)))+%2F+((1%2F(5+d+q))+%2B+(1-(1%2F(5+d+q)))+%2F+q)+%3C%3D+1+-+(1%2F(5+d+q))+q%5E-2%5
% So, $\|y_{t} - x^*\| \leq \Phi_{t} \|y_{t-1} - x^*\| \leq \Phi_{t} \|b_{t-1} - x^*\|$
%
So, it suffices to consider the case
\[\textstyle \zd{t-1} \geq \paren{\decayfactorq} R_{t-1}.\]
By Lemma~\ref{lem:prelim:radius_ratio}, $\zd{t-1} \leq \sqrt{Q} \bd{t-1} \leq \sqrt{\overline{Q}}\bd{t-1}$.
% it follows that $R_{t-1} \leq \paren{\decayfactor}\sqrt{Q} \bd{t-1}$.
Combined with our inductive hypothesis,
\(\textstyle \paren{\decayfactorq}\frac{1}{\sqrt{\overline{Q}}}R_{t-1} \leq \|b_{t-1} - x^*\| \leq R_{t-1}\)
and hence,
\[\textstyle \paren{\decayfactorq}\frac{1}{\overline{Q}\sqrt{\overline{Q}}}R_{t-1} \leq \frac{\|b_{t-1} - x^*\|}{Q} \leq R_{t-1}.\]
%
Our iteration over $k =0,\ldots, K$ sweeps through this range at an interval of size 1 in the $\log_2$ space, and combined with the multiplication in line \ref{alg:q:r}, it makes Theorem~\ref{thm:decay_probability} applicable.
Thus, each \emph{trial} has $\frac{1}{4}$ probability of producing a candidate for $b_t$ which would guarantee that
\begin{equation}
  \label{eq:qgld_induction}
  \textstyle
  \zd{t} \leq \paren{\decayfactor}R_{t-1} = R_t.
\end{equation}
%
By repeating $\log_{.75}\eta T^{-1} = \frac{\log (\eta^{-1} T)}{\log \frac{4}{3}} \leq 4 \log (\eta^{-1} T)$ trials, each epoch $t=1,\ldots,T$ fails to produce any candidate for $b_t$ to make Equation~\ref{eq:qgld_induction} hold with at most $\eta T^{-1}$ probability. By the union bound, this failure probability is at most $\eta$ over all epochs. So, the induction is valid with probabilty at least $1- \eta$.
\end{proof}
%
It follows that QGLD achieves the convergence rate of $O(\exp(-S / \log S))$.
 % where $S$ is the number of function evaluations.
\newcommand{\nuvalue}[0]{\ensuremath{\frac{\theta}{5 \dim}}}
\newcommand{\balnuvalue}[0]{\ensuremath{\frac{1}{5dQ^3}}}
\newcommand{\pevent}{\ensuremath{\rho}}
\begin{theorem}
Suppose that $\overline{Q}$ is no less than the condition number of $f$. Then, the output $b_T$ of QGLD satisfies with probability at least $1 - \eta$,
\[\textstyle \Phi(b_T) \leq \Phi(b_0) \exp\paren{-\frac{S}{40\dim \overline{Q}^3(\log_2 \overline{Q} +1)\log (\eta^{-1} S)}}.\]
\end{theorem}
If the upper bound $\overline{Q}$ is loose, then $R_t$ stays well above $\bd{t}$. As a result, QGLD tries to take very large steps that are unlikely to lead to any improvement.
On the other hand, if $\overline{Q} < Q$, then $R_t$ decreases faster than $\bd{t}$ and our algorithm will try to take small steps that are more likely to improve but only by a small amount. In practice, such slow but steady progress may be more desirable than all-or-zero progress, but our proof technique treat all small improvements below a certain threshold as zero improvement.


\subsection{\texorpdfstring{$\res$}{r}-Gradientless Descent}
\begin{algorithm}[t]
\SetKwBlock{Ballsample}{Ball Sampling Step:}{end}
\SetKwInOut{Input}{Input}
\caption{$\res$-GradientLess Descent ($\gamma$GLD) \label{alg:delta}}
  \Input{function $\obj: \R^\dim \to \R$, \\
  $T \in \Z_+$: number of evaluations of $f$, \\
  $\eta \in (0, 1)$: acceptable failure probability,  \\
  $\bp_0$: starting point, \\
  $\res$: resolution of the convergence}
  Set $K = \floor{\log{\frac{\|\X\|}{\res}}}$ and $R = \set{\frac{3}{5}\res \cdot 2^k : 0 \le k \le K}$ \\
  \For{$t = 1, \dots, T$}{
    Sample $\uar{r_t}{R}$ \\
    Sample $\uar{\candidate_t}{\cB(\bp_{t-1}, \frac{1}{ \sqrt{\dim}}r_t)}$.
    % , where
    % $B_t := \set{\point : \norm{x - \bp_{t-1}} \le r_t}$.
  % Set $\point_t$ to be the projection of $\candidate_t$ onto $\X$. \\
      %  Select $\point_t = \proj_{\X}\paren{\hat{\point}}$ to be the
      % projection of $\hat{\point}$ onto $\X$
\\
  \textbf{Update:}
    $\bp_t = \argmin \set{\obj(\point) : \point \in \set{\bp_{t-1}, \point_t}}$
     } % End For
\Return{$b_t$}
\end{algorithm}
$\res$GLD (Algorithm~\ref{alg:delta}) does not require any information about the objective function. Instead, it takes a resolution parameter $\res$ as input and its convergence guarantee only holds up to $Q \res$.
% This is more desirable in practice, because it is hard to obtain a tight upper bound on the condition number, and rather than fixing the number of evaluations, we often want to converge within a fixed error.
In other words, $\res$ is a lower bound on $\bd{t-1}/Q$ while the algorithm is still converging. For the upper bound, we use the trivial bound $\|\X\|$. 
% The main advantage of $\res$GLD over QGLD is that it does not require any information about the condition number as input, and the algorithm will still converge exponentially towards $Q \res$.

A big difference is that since $\res$GLD has no potential function to maintain, it is enough to take one random sample per iteration. Each iteration has a low probability of improving the function value significantly, but when we aggregate over a large number of iterations, we obtain a high probability bound.


\begin{theorem}
\label{thm:convergence_delta}
With probability at least $1 - \eta$, Algorithm~\ref{alg:delta} returns a point $x_T$ such that $f(x_T) -f(x^*) \leq \epsilon$ after $O(nQ \log(\|\X\|/\epsilon)^2)$ function evaluations.
\end{theorem}

\begin{proof}
By Theorem~\ref{thm:decay_probability}, as long as BLAH, the objective value will decrease multiplicatively by $1 - \frac{1}{5nQ}$ in each iteration. Therefore, we expect $f(x_T) -f(x^*) \leq \epsilon$ after $O(nQ\log(F/\epsilon))$ iterations, where $F = f(x_0) - f(x^*)$. Each iteration uses a binary search that requires $O(\log(\|\X\|/\epsilon))$ function evaluations. 

\end{proof}

The following theorem is somewhat misleading. Consider using the above theorem


\begin{theorem}
\label{thm:convergence_delta}
If $Q$ is the condition number of $f$, then with probability at least $1 - \eta$,
  \begin{equation*}
\bd{T} \le \max \paren{Q\res,
      \Phi_0 \paren{\decayfactor}^{\Lambda_T}
%      - \frac{\pevent (T-1) \bal \theta}{\dim \numradii}
%      + \sqrt{2 (T - 1) \balnuvalue \ln \paren{2 / \eta}}
        }
  \end{equation*}
where $\Lambda_T = \frac{T}{4 \log_2\paren{|\X| / \res}} - \sqrt{2 T \log \eta^{-1}}$.
\end{theorem}
% The above theorem shows that the algorithm converges exponentially towards $Q\res$.
% When the upper bound for $Q$ is known, we can optimize for $\res$ and $\res$GLD achieves the convergence rate of $O(\exp(-\sqrt{S}))$ where $S$ is the number of function evaluations, which is asymptotically slower than QGLD.
% \begin{corollary}
%  \label{thm:convergence_delta_Q}
%  Suppose there is an upper bound $\overline{Q}$ on the condition number of $f$.
%  Let $c = \log 2 / \log \paren{\decayfactorq}$ and set
% \[\gamma = \diam{\X}\paren{\decayfactorq}^{c\sqrt{\frac{T}{2\log\eta^{-1} + 2 c}}}.\]
% Then, the output $b_T$ of $\gamma$GLD satisfies
% \(\Phi(b_T) \leq Q\gamma\)
% % \exp\paren{-\frac{S}{40\dim Q^3(\log_2 Q +1)\log (\eta^{-1} S)}}\]
% with probability at least $1 - \eta$.
% \end{corollary}
\newcommand{\LLval}{Q^{-1}(1-\nu)}
\newcommand{\UUval}{\nu + Q^{-1}(1-\nu)}
\newcommand{\LL}{L}
\newcommand{\UU}{U}
  \newcommand{\azumavar}{}
  \newcommand{\az}{\ensuremath{z}}  % Quanity for Azuma's ineq.
% \begin{lemma}
% \label{lem:high_probability_bound}
% Suppose $f$ is a monotone transformation of a convex function with condition number $Q$. Then with probability at least $1-\eta,$
%   \begin{equation*}
%     { \bd{T} \le \max \paren{Q\res,
%       \Phi_0 \paren{\decayfactor}^{\Lambda_T}
% %      - \frac{\pevent (T-1) \bal \theta}{\dim \numradii}
% %      + \sqrt{2 (T - 1) \balnuvalue \ln \paren{2 / \eta}}
%         }
%       }
%      \end{equation*}
% where $\Lambda_T = \frac{T}{\log_2\paren{|\X| / \res}} - \sqrt{2 T \ln \eta^{-1}}$.
% \end{lemma}
  \begin{proof}
  Define $\Delta_t = \log_{\decayfactor}\frac{\Phi_{t}}{\Phi_{t-1}}$. Then, $\pot_T = \pot_0 \exp(\sum_{t=1}^T \Delta_T)$ and the theorem is a high-probability bound on the random variable $\Delta_{1:T} := \sum_{t=1}^T \Delta_t$. In order to apply concentration bounds, we define a bounded version of $\Delta_t$ as follows:
  \[
    \hdelta_t =
  \begin{cases}
    -1& \text{if $\Delta_t \leq -1$} \\
    0            & \text{otherwise.}
  \end{cases}
  \]
  Because our potential function never increases, $\Delta_t \leq \hdelta_t$ and
  it now suffices to upper bound the random variable $\hdelta_{1:T} := \sum_{t=1}^T \hdelta_t$.

  If $\bd{t} < Q\res$ for any $t \leq T$, then the statement is trivially true. So, assume $\bd{t} \geq Q\res$ for all $t$. Then, $\res \leq \frac{\bd{t}}{Q} \leq \diam{\X}$.
  Our choice of $R$ sweeps through this range with a unit-sized interval in the $\log_2$ space. Hence, we can apply Theorem~\ref{thm:decay_probability} and conclude there is at least $\frac{1}{4(K + 1)}$ probability that $\Delta_t \leq -1.$

 It immediately follows that
 \(\textstyle \expct{\hdelta_{1:T}} \ \le \ -\frac{T}{4 (K + 1)}.\)
  % \begin{split}
  % \expct{\hdelta_{1:T}} \le & -\sum_{t=1}^T \balnuvalue \pevent_t / \numradii \\
  % \le & -\frac{\pevent (T) \bal \theta}{\dim \numradii}
  % \end{split}
  % \end{equation*}
  Finally, we apply Azuma's inequality:
  \begin{equation} \label{eq:azuma1}
  \prob{ \hdelta_{1:T} - \expct{\hdelta_{1:T}} \geq \az }
  \le \exp \paren{-\frac{\az^2}{2T}}.
  \end{equation}
  To complete the proof, set
  $\az = \sqrt{2 T \log \eta^{-1}}$.
  \end{proof}
If we set $\res$ to be of order $\exp(-\sqrt{T}/\diam{\X})$, then $\Phi_T$ is of order $Q \exp\paren{-\frac{\sqrt{T} \log \eta^{-1}}{5\dim Q^3}}.$


\subsection{Optimistic QGLD}
% The optimistic QGLD uses small tweaks to enhance the performance of GLD. 
It is easy to see that $R_t$ in QGLD is an overly pessimistic upper bound on $\bd{t}$. In the proof of Lemma~\ref{lem:qgld}, we ignore all small improvements and use a uniform upper bound on the ratio $\frac{\Phi(b_{t})}{\Phi(b_{t-1})}$ no matter where exactly we land inside $\sublevelset_{q}$, which vastly underestimates the actual amount of improvements made.

In Figure~\ref{fig:bigq}, we tested the algorithms on $f_{1, Q, 20}$ for various values of $Q$. The results show that $R_t$ indeed vastly overestimates $\bd{t}$. After a few big successful steps in the beginning, QGLD stops making any progress while $R_t$ catches up to $\bd{t}$ at a very slow rate. Although $R_t$ should never underestimate $\bd{t}$ for our proof techniques to work, in practice it is preferable to keep $R_t$ close to $\bd{t}$ even if that means $R_t$ may underestimate $\bd{t}$.

We use slight modifications of QGLD to address this issue and make it use smaller step sizes. 
Optimistic QGLD uses
\begin{equation}
\label{eq:optimistic_radius}
\textstyle R_t = \diam{\X}\paren{1 - \frac{1}{5 \dim Q}}^{c_\dim t}
\end{equation}
where $c_\dim$ is the dimension-independent constant from Lemma~\ref{lem:ball-intersection}.
The biggest difference is that we drop the $Q^2$ factor from the denominator, because it is highly unlikely to see the worst-case of Lemma~\ref{lem:balanced} every time.
We multiply $t$ in the exponent by $c_\dim$, the constant in Lemma~\ref{lem:ball-intersection}.
So, $c_\dim t$ is the expected number of significant improvements up to iteration $t$.
Accordingly, we make only one trial as we no longer require every iteration to succeed with high probability. 
The last modification is that instead of iterating over all possible $k$ values, we use the largest possible $k$, which for QGLD is equivalent to using the smallest radius possible.

Back to Figure~\ref{fig:bigq}, we can see that the optimistic QGLD steadily converges, although for $Q=16$, optimistic QGLD is equivalent to assuming $256$ times more progresses than vanilla QGLD in computing $R_t$. This suggest that the actual decay rate is closer to Eq.~\ref{eq:optimistic_radius} than our theoretically provable bound for QGLD.

\section{Moved from ICLR version}
\begin{algorithm}[t]
\SetKwInOut{Input}{Input}
\caption{GradientLess Descent (GLD) \label{alg:gradientless}}
  \Input{function $\obj: \R^\dim \to \R$, \\
  $T \in \Z_+$: number of iterations, \\
  $x_0$: starting point, \\
  $\D$: sampling distribution \\}
  \For{$t = 0, \dots, T$}{
    Choose or sample a set of radii $\set{r_1,..,r_k}$. \\   
    Sample $v_1,..., v_k$ from $r_1\D, ..., r_k\D$. \\
  \textbf{Update:}
    $x_{t+1} = \arg \min_i \set{ f(y) \Big | \, y = x_t, \, y = x_t + v_i }$ \\
     } 
\Return{$x_t$}
\end{algorithm}



==> proofs.tex <==
%!TEX ROOT=aistats2019.tex
\newcommand{\LLval}{Q^{-1}(1-\nu)}
\newcommand{\UUval}{\nu + Q^{-1}(1-\nu)}
\newcommand{\LL}{L}
\newcommand{\UU}{U}

\section{Proofs}
\label{sec:proofs}

% We also define
% \[
% \pot(\point) := \paren{\max \set{\norm{y - \opt} : y \in \levelset_{\point)}},
% \]
% and the following shorthand notation:

\subsection{Step Size}
% For the vectors we define in this proof, we use the subscripts to denote the level set; for example, if a vector is named $a_t$, then it belongs to the level set $\levelset_{b_t}$.

% Suppose $\candidate_t \in B_q$, where $B_q$ is defined in Lemma~\ref{lem:goodevent}.
% Then, the update happens and $b_t \in \levelset_q$.

\begin{theorem}
\label{thm:decay_probability}
Suppose $\frac{3}{5} \frac{\xd{x}}{Q} \in [C_1, C_2]$ for some numbers $C_1, C_2 \in \R$. Then, there exist integers $0 \leq k_1, k_2 < \log\frac{C_2}{C_1}$ such that if $r = 2^{k_1} C_1$ or $r = 2^{-k_2} C_2$, then a random sample $y$ from uniform distribution over $B_x = \cB(x, r/\sqrt{\dim})$ satisfies
\[\textstyle \Phi(y) \leq \Phi(x) \paren{\decayfactor} \]
with probability at least $\frac{1}{4}$.

 % Let $R =\{r: r \leq C_2$ \text{ and } $r=2^k C_1$ for some non-negative integer $k\}$, or $R = \{r: r \geq C_1$ \text{ and } $r=2^{-k} C_2$ for some non-negative integer $k\}$. Then, there exists $r \in R$ such that
\end{theorem}
We first state the following simple corollary of Lemma~\ref{lem:prelim:radius_ratio}.
\begin{corollary}
\label{lem:potential_decay}
Let $\xx \in \X$ and $q = (1-\nuval)\xx + \nuval \point^*$. Then, for any $y \in \sublevelset_q$,
$\textstyle \Phi(y) \leq \Phi(x) \paren{\decayfactor}.$
\end{corollary}
Now we are ready to prove Theorem~\ref{thm:decay_probability}.
\begin{proof}
% , and $y$ be a random sample from uniform distribution over $B_x$.
Let $\nu = \frac{1}{5\dim\Q}$.
% Note that $\nu \leq 1/5$ for any $\Q, d \geq 1$.
Let $q = (1-\nu)\xx + \nu \point^*$.
Let $B_q = \cB(c_q, r_q)$ be a ball that has $q$ on its surface, lies inside $\sublevelset_q$, and has radius $r_q = Q^{-1}\|x - x^*\|$. Lemma~\ref{lem:enclosed_ball} guarantees its existence.

We will apply Lemma~\ref{lem:ball-intersection} to show that at least $\frac{1}{4}$ fraction of $B_x$ is contained in $B_q$; the theorem statement then follows from Corollary~\ref{lem:potential_decay}.  It remains to show that the radius of $B_x$ and $B_q$ are in the required range for Lemma~\ref{lem:ball-intersection}.

Let $\ell = \norm{x - c_q}$.
Note that
\begin{align}
\ell &\leq \|\xx - q\| + r_q \label{eq:ell_rq}\\
&\leq \nu \xd{\xx} + r_q  = \nu \xd{\xx} + Q^{-1} \xd{q} \notag \\
&\leq \textstyle (\nu + Q^{-1}(1-\nu))\xd{x} \leq \frac{6}{5Q}\bd{x}. \label{eq:ell_lx}
% &\leq \textstyle  \label{eq:ell_lq}
\end{align}
Since $\xx$ is outside of $B_q$, we also have
\begin{align}
\ell &\geq r_q = Q^{-1}\xd{q} = Q^{-1}(1-\nu)\xd{\xx} \notag \\
& \textstyle \geq \frac{4}{5Q}\bd{x}. \label{eq:ell_ux}
\end{align}
% Define shorthand notations $\LL = \LLval$ and $\UU = \UUval$, so that we can write $\LL \xd{\xx} \leq \ell \leq \UU \xd{\xx}.$

So, $\frac{\ell}{2} \leq \frac{3}{5Q}\bd{x}  \leq \ell$.
\textbf{(TODO: improve wording here)}
The logarithmic swap through $[C_1, C_2]$ therefore guarantees that
There exists $r \in R$ such that
\(\textstyle r \in [\ell/2, \ell].\)

Now we will show that \(r_q \geq (1 - 1/(4 \dim))\ell.\)
From Eq. \eqref{eq:ell_lx}, it suffices to prove that $\|x - q\| \leq \frac{\ell}{4\dim}$ or equivalently $\nu\xd{\xx} \leq \frac{\ell}{4\dim}$. From Eq. \eqref{eq:ell_ux},
\[\|x - q\| = \nu \xd{\xx} \leq \nu Q(1-\nu)^{-1}\ell.\]
For any $\Q, \dim \geq 1$, $1 - \nu \geq \frac{4}{5}$. So,
\begin{equation}
\label{eq:good_event:1}
\textstyle
  \nu Q(1-\nu)^{-1} = \frac{1}{5\dim}(1 - \nu)^{-1}\leq \frac{1}{4\dim}
\end{equation}
and the proof is complete.
\end{proof}

\todo[inline]{handle projections more carefully}

\begin{lemma}
\label{lem:ball-intersection}
  Let $B_1$ and $B_2$ be two balls in $\R^\dim$ of radii $r_1$ and $r_2$ respectively.
  Let $\dc$ be the distance between the centers.
  If $r_1 \in [\frac{\dc}{2\sqrt{\dim}}, \frac{\dc}{\sqrt{\dim}}]$ and
  $r_2 \ge \dc - \frac{\dc}{4 \dim}$, then
  \[
   \vol{B_1 \intersect B_2} \geq c_\dim \vol{B_1},
  \]
  where $c_\dim$ is a dimension-dependent constant that is lower bounded by $\ballconst$ at $\dim = 1$.
\end{lemma}
\begin{proof}
It suffices to prove for the unit distance case $\ell = 1$, and $r_2 = 1 - \frac{1}{4 \dim}$, because
  $\vol{B_1 \intersect B'} \le \vol{B_1 \intersect B}$ whenever $B' \subset B$.


Since $|r_1 - r_2| \leq \dc \leq r_1 + r_2$, the intersection $B_1 \intersect B_2$ is composed of two hyperspherical caps glued end to end.
We lower bound $\vol{B_1 \intersect B_2}$ by the volume of the cap $C_1$ of $B_1$ that is contained in the intersection.
Consider the triangle with sides $r_1, r_2$ and $\dc$.
From classic geometry,
  \begin{equation} \label{eq:cap-height}
    % c_1 = \frac{\dc}{2}\paren{1 + r_1^2 - r_2^2} > 0.
    c_1 = \frac{1}{2}\paren{1 + r_1^2 - r_2^2}
    =
     > 0.
  \end{equation}
The volume of a spherical cap is \cite{li2011concise},
\[\vol{C_1} = \frac{1}{2} \vol{B_1} I_{1 - \frac{c_1^2}{r_1^2}}(\frac{n+1}{2}, \frac{1}{2}).\]
where $I$ is the regularized incomplete beta function defined as
\[I_x(a,b) = \frac{\int_{0}^{x} t^{a-1} (1 - t)^{b-1} \ dt}{\int_{0}^{1} t^{a - 1} (1 - t)^{b-1} \ dt} \]
where $x \in [0,1]$ and $a,b \in (0, \infty)$.
Note that for any fixed $a$ and $b$, $I_x(a,b)$ is increasing in $x$.
Hence, in order to obtain a lower bound on $\vol{C_1}$, we want to lower bound
$1 - \frac{c_1^2}{r_1^2}$
or equivalently, upper bound $\frac{c_1^2}{r_1^2}.$

  Write $r_1 = \frac{\alpha}{2\sqrt{\dim}}$ for some $\alpha \in [1,2]$.
  % We will show $c_1 \le \frac{3 r_1}{4\sqrt{\dim}}$ for all $\alpha \in [1, 2]$.
  % or equivalently, $r_1 / \sqrt{\dim} - c_1 \ge 0$.
  From \eqr{cap-height},
  \[
    c_1 = \frac{1}{4\dim} + \frac{\alpha^2}{8\dim} - \frac{1}{32\dim^2}.
  \]
  Hence,
  \[
  \frac{c_1}{r_1} = \frac{1}{16\sqrt{\dim}}\paren{\frac{8}{\alpha} + 4\alpha - \frac{1}{\dim}}
  \]
  Since $g(\alpha) = \frac{8}{\alpha} + 4\alpha$ is convex in $[1,2]$, $g(\alpha) \leq \max(g(1), g(2)) = 12.$ It follows that $\frac{c_1}{r_1} \leq \frac{1}{16\sqrt{\dim}}\paren{12 - \frac{1}{\dim}} \leq \frac{3}{4 \sqrt{\dim}}.$
So, $1 - \frac{c_1^2}{r_1^2} \geq 1 - \frac{16}{9\dim}.$ To complete the proof,
note that
$V_\dim := I_{1 - \frac{16}{9\dim}}(\frac{\dim + 1}{2}, \frac{1}{2})$ is increasing in $\dim$, and $V_1 = \ballconst$. As $\dim$ goes to infinity, this value converges to $1$ as $B_1 \subset B_2$.
% This last bit is proof by mathematica:
% http://www.wolframalpha.com/input/?i=Plot%5BBetaRegularized%5B1-1%2Fn,+(n%2B1)%2F2,+1%2F2%5D,+%7Bn,2,1000%7D%5D
\end{proof}

\subsection{Convergence of Q-Gradientless Descent}
\begin{lemma}
For QGLD, $\Phi_t \leq R_t$ for all $t$ with probability $1 - \eta$.
\end{lemma}
\begin{proof}
Let $z_t = \arg\max_{x: f(x) = f(b_t)} \|x - x^*\|$ be the point in $\levelset_{b_t}$ that is maximally far from $x^*$.
Clearly, $\zd{0} \leq R_0 = \diam{\X}$. Now suppose $\zd{t-1} \leq R_{t - 1}$ for induction.

% Let $q = \paren{\decayfactor}\bp_{t-1} + \frac{1}{5d\Q} \point^*$.
% Let $B_q = \cB(c_q, r_q)$ be ball contained in $\levelset_q$ such that $q$ is on its surface; the existence of $B_q$ is guaranteed by Lemma~\ref{lem:enclosed_ball}.

% % Let $\nu = \nuval.$

% Let $\ell = \|b_{t-1} - c_q\|$. Note that
% \begin{equation}
%   \frac{\UU}{\LL} = 1 + \nu Q(1-\nu)^{-1} = 1 + \frac{1}{5\dim}(1 - \nu)^{-1}
% \leq 1 + \frac{1}{4 \dim} \leq \frac{5}{4}
% \end{equation}
% and
% \begin{equation}
% \frac{L}{U} \leq \decayfactor
% \end{equation}
% for all $\dim, Q \geq 1.$

If $\|z_{t-1} - x^*\| \leq \paren{\decayfactorq} R_{t-1}$, then we trivially have:
% $ \|z_{t-1} - x^*\| < \frac{\LL}{\UU}R_{t-1} \leq (1-\frac{1}{5 \dim Q^3}) R_{t-1} = R_t$ and therefore
 \(\bd{t} \leq \|z_{t} - x^*\| \leq \|z_{t-1} - x^*\| \leq  R_{t}.\)
%
% \textbf{Case 2:} Suppose $\LL\|b_{t-1} - x^*\| \leq \LL\Phi_{t-1} \leq \UU \|b_{t-1} - x^*\|$.
% Note that $\ell$ also belongs to this interval and $\frac{\LL}{\UU} \geq \frac{4}{5}$. If $\hat{\ell}\leq \ell$, then $\hat{\ell} \geq \frac{4}{5} \ell \geq ell/2.$ Otherwise, $\ell \leq \hat{\ell}$ but $\ell \geq  \frac{4}{5}\hat{\ell}$ and also, $\ell/2 \leq \frac{4}{5}\ell \leq \frac{4}{5}\hat{\ell}$. Therefore,
%  at least one of $\hat{\ell}$ or $\frac{4}{5}\hat{\ell}$ is in $[\ell/2, \ell]$.
% %Proof by mathematica: http://www.wolframalpha.com/input/?i=Solve%5Bq%5E-1+(1-+(1%2F(5+d+q)))+%2F+((1%2F(5+d+q))+%2B+(1-(1%2F(5+d+q)))+%2F+q)+%3C%3D+1+-+(1%2F(5+d+q))+q%5E-2%5
% So, $\|y_{t} - x^*\| \leq \Phi_{t} \|y_{t-1} - x^*\| \leq \Phi_{t} \|b_{t-1} - x^*\|$
%
So, it suffices to consider the case
\[\textstyle \zd{t-1} \geq \paren{\decayfactorq} R_{t-1}.\]
By Lemma~\ref{lem:prelim:radius_ratio}, $\zd{t-1} \leq \sqrt{Q} \bd{t-1} \leq \sqrt{\overline{Q}}\bd{t-1}$.
% it follows that $R_{t-1} \leq \paren{\decayfactor}\sqrt{Q} \bd{t-1}$.
Combined with our inductive hypothesis,
\[\paren{\decayfactorq}\frac{1}{\sqrt{\overline{Q}}}R_{t-1} \leq \|b_{t-1} - x^*\| \leq R_{t-1}\]
and hence,
\[\paren{\decayfactorq}\frac{1}{\overline{Q}\sqrt{\overline{Q}}}R_{t-1} \leq \frac{\|b_{t-1} - x^*\|}{Q} \leq R_{t-1}\]


Our iteration over $k =0,\ldots, K$ guarantees that we do a logarithmic sweep through this range, and the multiplication in line \ref{alg:q:r} makes Theorem~\ref{thm:decay_probability} applicable. Thus, each \emph{trial} has $\frac{1}{4}$ probability of producing a candidate for $b_t$ which would guarantee that
\begin{equation}
  \label{eq:qgld_induction}
  \zd{t} \leq \paren{\decayfactor}R_{t-1} = R_t.
\end{equation}

By repeating $\log_{.75}\eta T^{-1} = \frac{\log (\eta^{-1} T)}{\log \frac{4}{3}} \leq 4 \log (\eta^{-1} T)$ trials, each epoch $t=1,\ldots,T$ fails to produce any candidate for $b_t$ to make Equation~\ref{eq:qgld_induction} hold with $\eta T^{-1}$ probability. By the union bound, this failure probability is only $\eta$ over all epochs. So, the induction is valid with probabilty at least $1- \eta$.
\end{proof}


\subsection{Convergence of \texorpdfstring{$\res$}{r}-GLD}

  \newcommand{\azumavar}{}
  \newcommand{\az}{\ensuremath{z}}  % Quanity for Azuma's ineq.
\begin{lemma}
\label{lem:high_probability_bound}
Suppose $f$ is a monotone transformation of a convex function with condition number $Q$. Then,
  \begin{equation*}
    \prob{ \bd{T} \le \max \paren{Q\res,
      \Phi_0 \paren{\decayfactor}^{\Lambda_T}
%      - \frac{\pevent (T-1) \bal \theta}{\dim \numradii}
%      + \sqrt{2 (T - 1) \balnuvalue \ln \paren{2 / \eta}}
        }
      }
    \le 1 - \eta.
  \end{equation*}
where $\Lambda_T = \frac{T}{\log_2\paren{|\X| / \res}} - \sqrt{2 T \ln \eta^{-1}}$.
\end{lemma}
  \begin{proof}
  Define $\Delta_t = \log_{\decayfactor}\frac{\Phi_{t}}{\Phi_{t-1}}$. Then, $\pot_T = \pot_0 \exp(\sum_{t=1}^T \Delta_T)$ and the theorem is a high-probability bound on the random variable $\Delta_{1:T} := \sum_{t=1}^T \Delta_t$. In order to apply concentration bounds, we define a bounded version of $\Delta_t$ as follows:
  \[
    \hdelta_t =
  \begin{cases}
    -1& \text{if $\Delta_t \leq -1$} \\
    0            & \text{otherwise.}
  \end{cases}
  \]
  Because our potential function never increases, $\Delta_t \leq \hdelta_t$ and
  it now suffices to upper bound the random variable $\hdelta_{1:T} := \sum_{t=1}^T \hdelta_t$.

  If $\bd{t} < Q\res$ for any $t \leq T$, then the statement is trivially true. So, assume $\bd{t} \geq Q\res$ for all $t$. Then, $\res \leq \frac{\bd{t}}{Q} \leq \diam{\X}$.
  Our choice of $K$ guarantees that the candidate radius set $R$ is a logarithmic sweep through this range. Hence, by Theorem~\ref{thm:decay_probability}, there is at least $\frac{1}{4(K + 1)}$ probability that $\Delta_t \leq -1.$

 It immediately follows that
 \(\textstyle \expct{\hdelta_{1:T}} \ \le \ -\frac{T}{4 (K + 1)}.\)
  % \begin{split}
  % \expct{\hdelta_{1:T}} \le & -\sum_{t=1}^T \balnuvalue \pevent_t / \numradii \\
  % \le & -\frac{\pevent (T) \bal \theta}{\dim \numradii}
  % \end{split}
  % \end{equation*}
  Finally, we apply Azuma's inequality:
  \begin{equation} \label{eq:azuma1}
  \prob{ \hdelta_{1:T} - \expct{\hdelta_{1:T}} \geq \az }
  \le \exp \paren{-\frac{\az^2}{2T}}.
  \end{equation}
  To ensure this probability is at most $\eta$, it suffices to set
  $\az = \sqrt{2 T \ln \eta^{-1}}$, which completes the proof.
  \end{proof}

% \input{nodelta_proof}

